Parameterized Yang-Hilbert-Type Integral Inequalities and Their Operator Expressions

Applying methods of Real Analysis and Functional Analysis, we build two weight functions with parameters and provide two kinds of parameterized Yang-Hilbert-type integral inequalities with the best constant factors. Equivalent forms, the reverses, and the operator expressions are also given. In particular, the Hardy-type inequalities and Hardy-type operators are studied. Additionally, a number of examples with two kinds of particular kernels are considered.

==> cblist.tex <==
%%%%%%%%%%%%%%%%%%%% file editor.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% sample file for a complete "list of contributors"
%
% Copy it to a new file with a new name and
% use it as a template for your own input.
%
% please note that this environment makes use of the
% "obeylines"-function.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thecontriblist}
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*} \and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*} \and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\and
\textbf{Author Name}
University/Institute Name
Street No.
X - Place, Postal Code
\texttt{name@e-mail.*}
\end{thecontriblist}


==> dedic.tex <==

%%%%%%%%%%%%%%%%%%%%%%% dedic.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% sample dedication
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

\thispagestyle{empty}
\vspace*{3.5cm}
\begin{flushright}

% write your text here
{\large Your dedication goes here}

\end{flushright}





==> part.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample part title
%
% Copy it to a new file with a new name and use it
% use it as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%


\part{Part Title}


==> pref.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample preface
%
% Copy it to a new file with a new name and use it as the basis
% for your article
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

\preface

%% Please write your preface here
Here come the golden words

\vspace{1cm}
\begin{flushright}\noindent
place(s),\hfill {\it Firstname  Surname}\\
month year\hfill {\it Firstname  Surname}\\
\end{flushright}




==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
%
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
% Non-BibTeX users please use
\begin{thebibliography}{[KLR73]}
%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references
%
% Monographs
\bibitem[KLR73]{monograph} Kagan, A.M., Linnik, Y.V., Rao, C.R.:
Characterization Problems in Mathematical Statistics. Wiley, New York (1973)

% Contributed Works
\bibitem[Mey89]{contribution} Meyer, P.A.: A short presentation of
stochastic calculus. In: Emery, M. (ed) Stochastic Calculus in
Manifolds. Springer, Berlin Heidelberg New York (1989)

% Journal
\bibitem[MR97]{journal} Miller, B.M., Runggaldier, W.J.: Kalman
filtering for linear systems with coefficients driven by a hidden Markov
jump process. Syst. Control Lett., \textbf{31}, 93--102 (1997)

% Theses
\bibitem[Ros77]{thesis} Ross, D.W.: Lysosomes and storage diseases. MA
Thesis, Columbia University, New York (1977)

\end{thebibliography}

